Edge to Cloud Tools: A Multivocal Literature Review

Edge-to-cloud computing is an emerging paradigm for distributing computational tasks between edge devices and cloud resources. Different approaches for orchestration, offloading, and many more purposes have been introduced in research. However, it is still not clear what has been implemented in the industry. This work aims to merge this gap by mapping the existing knowledge on edge-to-cloud tools by providing an overview of the current state of research in this area and identifying research gaps and challenges. For this purpose, we conducted a Multivocal Literature Review (MLR) by analyzing 40 tools from 1073 primary studies (220 PS from the white literature and 853 PS from the gray literature). We categorized the tools based on their characteristics and targeted environments. Overall, this systematic mapping study provides a comprehensive overview of edge-to-cloud tools and highlights several opportunities for researchers and practitioners for future research in this area.

==> Sections/Discussion_Backup.tex <==
\section{Discussion}
\label{sec:Discussion}

Given the hype that has targeted cloud computing for more than a decade, as expected, most tools target the execution of tasks on the cloud. 


Only  2 tools target actual offloading of tasks being executed, which is clearly a consequence of the  inherent technical hurdles that are involved in such a process. Only 2 tools are able to perform as workflow managers. On the other hand,  many more tools are able to perform orchestration, thus deciding where to execute at task as the task is launched.



Kubernetes is heavily represented. Cloud native == OCI dominating, only two in proprietary container.

End to end tools primarily by very big companies. Ormuco is the only exception to this rule, being a company employing 34 people only (2022 data).


Only one simulator. Are things analyzed primarily at run-time for live systems with less consideration of how different scenarios could play out?

Regarding target platforms: platform agnostic ones are the most common. the closer you move to hw the more difficult it gets to support heterogeneous hardware/software platforms which can also be seen by only few targeting mainly edge nodes, and only one for the far edge.

\subsection{Feature challenges}

The analysis of the literature shows that the design of systems allowing for task offloading is still in its infancy. In fact, the tools are either targeted at a specific use case or are extensions of mainstream tools such as Kubernetes or containers. Moreover, the lack of interest in simulation hints that the scenarios under consideration are limited in size. 

To cover targeted use cases, most tools are either providing coverage for end-to-end service, or are full software platforms. This approach works against standardization and interoperability efforts, which would grow if it was possible to use different tools for the different actions related to task offloading and orchestration. 


\subsection{Threats to validity}


We are aware that our work is subject to threats to validity, since we got through only tools that are available either commercially or as OSS, while other tools could be used internally by large companies, or more advanced techniques could be being developed and close to reach the maturity level required to be part of a tool such as the ones included in this analysis.

One more issue, that we tried to solve with a thorough analysis, was that some tools could have been abandonded, and slowly growing obsolescent. 

With regards to the tools' features, we based our analysis on the material available as bibliography, and on the tools' website, not considering experimental features. This approach can be too defensive and produce a number of false negatives, still we preferred this issue than to accept characteristics and capabilities not mature enough for a tools that can be used in a production environment.


To improve the reliability of this work, we defined search terms and applied procedures that can be replicated by others. Since this is a mapping study and no systematic review, the inclusion/exclusion criteria are only related to whether the topic of Cognitive Cloud is present in a paper or not, as suggested by~\cite{petersen2008systematic}. 

As for the analysis procedure, since  our analysis only uses descriptive statistics, the threats are minimal. However, we are aware that the synthesis of the definition might be subjective. To mitigate this threat, the analysis was done collaboratively, using a collecting coding method, and discussing with all the authors about inconsistencies. The Kohen K index about our disagreement also confirms the quality of the qualitative analysis performed. 



==> Sections/Study_Design_Backup.tex <==
\section{Study Design}
\label{sec:ResearchDesign}

This section outlines the process used for this work, which involved a Multivocal Literature Review (MLR) following the guidelines proposed by Garousi et al.~\cite{Garousi18a}, due to the topic's novelty. The following subsections provide a summary of the MLR process, including selection of primary studies, quality assessment of the gray literature, data extraction, tools selection, conducting the review and varifiability and replicability.

    
\subsection{MLR process overview}  
The MLR process encompasses a variety of sources, including peer-reviewed and gray literature, and acknowledges the diverse perspectives of both practitioners and academic researchers. To categorize contributions, MLR distinguishes between academic literature (peer-reviewed papers) and gray literature (other forms of content such as blog posts, white papers, podcasts, etc.).

%The MLR process is composed of four steps, as depicted in Figure \ref{fig:mlrprocess}:
%\begin{itemize}
    %\item \textit{Selection of primary studies} from the gray and white literature;
    %\item \textit{Quality Assessment} of the selected gray literature; 
    %\item \textit{Data extraction} of the information needed to answer our RQs;
%\begin{itemize}
    %\item Data Extraction from the primary studies 
    %\item Data Extraction from the tools' websites
%\end{itemize}
%\item \textit{Tools Selection } 
%\item \textit{Data synthesis} of the extracted results 
%\end{itemize}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/PLOTProcess.pdf}
    \caption{Overview of the followed MLR process}
    \label{fig:mlrprocess}
\end{figure}

\subsection{Selection of Primary Studies}
\label{sec:Selection}
The first step for selecting the Primary Studies (PS) is the search string identification that will be adopted in the academic bibliographic sources and in the gray literature source engines. 
We define the search string as follow:

\begin{center}
\textbf{("edge cloud" OR "edge-to-cloud") \\
AND \\
(offloading OR cognitive OR orchestration) \\
AND\\
tool}
\end{center}
%
To maximize the number of works identified, the search terms were used across all fields (i.e. title, abstract, and keywords). The same search terms were utilized for both gray literature from online sources and white literature from academic bibliographic sources, with both searches being performed in November 2022.

\textbf{Peer-reviewed literature search}. We considered the papers indexed by five bibliographic sources:


\begin{itemize}
    \item IEEEXplore digital library \cite{ieee}
    \item Scopus \cite{scopus}
    \item ACM digital library \cite{acm}
    \item Science Direct \cite{sciencedirect}
    \item ISI Web of science \cite{webofscience}
\end{itemize}


\textbf{Gray literature search}. 
%Also, in this case, we extended the search to a wider set of search engines compared to~\cite{Recupito2022}. Therefore, 
We performed the search using two search engines: 

\begin{itemize}
    \item Google Search\footnote{\url{https://www.google.com/}} 
    %\item Twitter\footnote{\url{https://twitter.com/}}
    %\item Reddit\footnote{\url{https://www.reddit.com/}} 
    \item Medium\footnote{\url{https://medium.com}}
\end{itemize}

The search results consisted of books, blog posts, forums, websites, videos, white-paper, frameworks, and podcasts. 
 

\textbf{Snowballing}. Snowballing involves utilizing the references or citations of a paper to identify additional primary studies \cite{wohlin2014guidelines}. In this work, backward snowballing was employed for the academic literature to identify relevant primary studies from the references of selected sources. Additionally, backward snowballing was applied to the gray literature by following outgoing links of each selected source.

\textbf{Application of inclusion and exclusion criteria}. Based on guidelines for Systematic Literature Reviews \cite{keele2007guidelines}, we defined \textit{inclusion and exclusion} criteria (Table \ref{tab:inclusionExclusion}). 
We considered less restrictive inclusion criteria to enable the inclusion of a more comprehensive set of tools.

To ensure the effectiveness of the inclusion and exclusion criteria, a subset of 10 randomly selected primary studies (PSs) from those retrieved were tested prior to their application. The resulting inclusion and exclusion criteria are outlined in Table~\ref{tab:coding}.

To screen each paper, two researchers were tasked with independently reviewing them in a fair manner. The paper assignments were mixed up and each researcher was given a similar number of papers to review, along with other team members. In case of disagreements, a third author was consulted to arrive at a consensus and improve the reliability of the study. Before involving the third author, Cohen's kappa coefficient was calculated to assess inter-rater agreement. The results of this assessment can be found in the replication package~\footref{Package}.

\begin{table}[h]
\centering
\footnotesize
    \caption{Inclusion/Exclusion Criteria for Selection }
    \label{tab:coding}
    \begin{tabular}{l|p{5.3cm}}
    \hline 
\textbf{Primary Study (PS)} & \textbf{Criteria}\\ \hline
\multirow{1}{*}{\textbf{Inclusion}} & Research papers or search results that are mentioning edge-to-cloud offloading tools and their characteristics\\ \hline
\multirow{1}{*}{\textbf{Exclusion}} & - Not in English  \\

\hline 
\textbf{Tools Selection} & \textbf{Criteria}\\ \hline
\multirow{1}{*}{\textbf{Inclusion}} & Commercial and Open Source Tools \\\hline
\multirow{1}{*}{\textbf{Exclusion}} & - Not downloadable  \\
\multirow{1}{*}{\textbf{Exclusion}} & - Open Source Tools with less than 100 stars in GitHub\\\hline

\end{tabular}
%\vspace{0.2cm}
\label{tab:inclusionExclusion}
\end{table}


\subsection{Quality Assessment of the Gray Literature}
\label{sec:Quality}
In contrast to peer-reviewed literature, gray literature is not subjected to a formal review process and its quality is less regulated. In order to assess the credibility and quality of selected gray literature sources and determine whether or not to include them, we followed the guidelines recommended by Garousi et al.~\cite{Garousi18a}, taking into account the authority of the producer, applied methodology, objectivity, date, novelty, and impact.

To evaluate each source, the first two authors utilized the aforementioned criteria, using either a binary or three-point Likert scale depending on the specific criteria. In cases of disagreement, the evaluation was discussed with the third author, who provided a third opinion, and discussed with the two original evaluators until disagreements are solved.

\subsection{Data Extraction}
As our goal is to characterize information from edge-to-cloud offloading tools, we need to get these pieces of information directly from the tools' websites. 
Therefore, the data extraction process is composed of two steps: 
%the extraction of the list of tools from the PS, and then the extraction of the information on the tools from their websites. 
% \subsubsection{Data Extraction from the Primary Studies (Preliminary Tools List)}
% \label{sec:toolextraction}
% The extraction process was composed by two main steps: 
\begin{itemize}
    \item[(PE)]\textit{Extraction of the list of tools from the primary studies} (PSs) that satisfied the quality assessment criteria. 
    \item[(TE)] \textit{Extraction of the information from the tools list}. In this case, we extracted the information directly from the official website portals.
\end{itemize}

We utilized a review spreadsheet to extract information in accordance with our research questions (RQs). A summary of the data extraction form, as well as the mapping of necessary information for addressing each RQ, can be found in Table~\ref{tab:ext}.

\todo[inline]{I need help to make the list of information we extracted for each tool}
\begin{table}[]
  \footnotesize
    \centering
    \caption{Data Extraction }
    \label{tab:ext}
    \begin{tabular}{l|l|p{4.2cm}|l} \hline
\textbf{RQs}	& 	\textbf{Info}	&	\textbf{Description}	& \textbf{Step	}\\
\hline
\end{tabular}
\end{table}

The data extraction process adhered to the qualitative analysis guidelines put forth by Wohlin et al.~\cite{wohlin2012experimentation}. All information was extracted by two researchers. If there was disagreement, a third author was consulted and a discussion was held until the disagreement was resolved.

\subsection{Tool Selection}
To identify the final set of tools required to answer our RQs, a similar process to the one employed in the paper selection phase (Section~\ref{sec:Selection}) was applied, which involved filtering the tools based on a set of inclusion and exclusion criteria.

As with the PS selection process, we tested the applicability of the inclusion and exclusion criteria on a randomly selected subset of 10\% of the retrieved tools before applying them. The final set of inclusion and exclusion criteria is presented in Table \ref{tab:inclusionExclusion}.

The tool selection was carried out by two researchers who independently reviewed them, as was the case with the PS selection. In the event of any discrepancies, a third author was brought in to reach a consensus. The inter-rater agreement was also assessed in this case by calculating Cohen's kappa coefficient. These results are documented in the replication package~\footref{Package}.

\subsection{Conducting the review}

From the Search process, conducted in November 2022, we retrieved a total of 1104 unique PS (after the exclusion of 137 duplicated): 854 PS from the gray literature (Table~\ref{tab:grayResults}) and 250 PS from the white literature (Table~\ref{tab:bibliographicResults}). The snowballing process enabled to include XX more sources (XXX from white literature and XXX from gray literature). 

255 PS (51 from white literature, 204 from gray literature) were selected after applying inclusion and exclusion criteria, with an almost perfect agreement (Cohen's kappa = 0.869). 

The quality assessment process on gray literature PS excluded XX papers, leading to a total of XXX PS (XXX from gray literature, XXX from white literature). 

From the data extraction process, 338 tools were obtained. 

The application of inclusion and exclusion criteria for tools resulted in almost perfect agreement (Cohen's kappa = XXX) and a final set of 94 tools , as reported in Table \ref{tab:selectedTools}.
\todo[inline]{(BEFORE QUALITY)}
\begin{table}[h] 
\caption{Initial search result from bibliographic sources.}
\begin{tabular}{lc}
\hline
\multicolumn{1}{c}{\textbf{Bibliographic Source}} & \textbf{\#non-duplicated papers} \\
\hline
IEEEXplore                             & 5                                        \\
Scopus                                 & 150                                      \\
ACM Digital Library                    & 81                                       \\
Science Direct                         & 1                                        \\
ISI Web of Science                     & 13                                       \\\hline
\textbf{Total}              & 250                             \\\hline
\hline
\end{tabular}
\label{table:bibliographicResults}
\end{table}


\begin{table}[h]
\caption{Search results from Gray Literature Search Engines.}
\begin{tabular}{lc}
\hline
\multicolumn{1}{c}{\textbf{Search engines}} & \textbf{\#non-duplicated search result} \\
\hline
Google search                              & 495                                         \\
Medium search                              & 359                                   \\\hline
\textbf{Total}         & \textbf{854}                                             \\\hline
\hline
\end{tabular}
\label{table:2}
\end{table}


\subsection{Verifiability and Replicability}
\noindent To allow our study to be replicated, we have published the complete raw data in the replication package.\footnote{\url{LINK}\label{Package}}.



% A systematic Multivocal Literature Review includes academic literature (e.g. papers that published in journals, conferences, workshops) and grey literature (e.g. white papers, blog posts). While the MLRs provide the summaries from both academic and grey literature,  they are useful for both researchers and practitioners \cite{Garousi18a}. 
% We processed the MLR based on these steps:

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.4\textwidth]{Figures/PLOTProcess.pdf}
%     \caption{Overview of the followed MLR process (adapted from Fig. 7 in \cite{Garousi18a})}
%     \label{fig:mlrprocess}
% \end{figure}

% \begin{itemize}
% \item Selecting the keywords based on the research questions
% \item Selecting the key sources to start the initial search
% \item Study the material
% \item Defining a selection strategy
% \item Data extraction and synthesis
% \item Creating the final results
% \end{itemize}

% The detailed process is illustrated in (Figure~\ref{fig:mlrprocess}).

% \subsection{Search strategy}  

% In this section, first we describe the process of searching for the academic literature and then the strategy we adopted for the grey literature.

% \subsubsection{Academic literature search}

% The traditional systematic literature review has been adopted for the academic literature in this work. \\
% First we selected these 5 common digital libraries, namely:

% \begin{itemize}
%     \item IEEEXplore digital library \cite{ieee}
%     \item Scopus \cite{scopus}
%     \item ACM digital library \cite{acm}
%     \item Science Direct \cite{sciencedirect}
%     \item ISI Web of science \cite{webofscience}
% \end{itemize}

% We defined search strings to query on the mentioned digital libraries as follows:


% \begin{center}
% \textbf{("edge cloud" OR "edge-to-cloud") \\
% AND \\
% (offloading OR cognitive OR orchestration) \\
% AND \\
% tool}
% \end{center}
% %

% We conducted our search in September 2022, extracting 250 non-duplicated papers from the libraries mentioned above. Table \ref{table:1} reports the number of papers for each libraries. \\

% \begin{table}[h] 
% \caption{Initial search result from libraries.}
% \begin{tabular}{lc}
% \hline
% \multicolumn{1}{c}{\textbf{Libraries}} & \textbf{Number of non-duplicated papers} \\
% \hline
% IEEEXplore                             & 5                                        \\
% Scopus                                 & 150                                      \\
% ACM Digital Library                    & 81                                       \\
% Science Direct                         & 1                                        \\
% ISI Web of Science                     & 13                                       \\
% \multicolumn{1}{c}{\textbf{Total}}              & 250                             \\
% \hline
% \end{tabular}
% \label{table:1}
% \end{table}

% \subsubsection{Grey literature search}

% For retrieving grey literature, we adopted the same search string. We applied them into 2 search engines which are Google search and Medium search. These searches were performed in September and October 2022 and the search results were copied to a Spreadsheet. Table \ref{table:2} reports the number of search results for each search engine.\\

% \begin{table}[h]
% \caption{Initial search result from search engines.}
% \begin{tabular}{lc}
% \hline
% \multicolumn{1}{c}{\textbf{Search engines}} & \textbf{Number of non-duplicated search result} \\
% \hline
% Google search                              & 496                                             \\
% Medium search                              & 359                                             \\
% \multicolumn{1}{c}{\textbf{Total}}         & 855                                             \\
% \hline
% \end{tabular}
% \label{table:2}
% \end{table}


% \subsection{Selection strategy} 
% The primary search results were shortlisted by defining the inclusion and exclusion criteria for our study. We defined them as:
% \begin{itemize}
%     \item Inclusion criteria 1: Research papers or search results that are mentioning edge-to-cloud offloading tools and their characteristics
%     %\item Exclusion criteria 1: Results that mentioned about edge-to-cloud- offloading simulators, algorithms or the ones for testing
%     \item Exclusion criteria 1: Results that are not in English
%     \item Exclusion criteria 2: Duplicated results
% \end{itemize}

% Following the defined inclusion and exclusion criteria, we evaluated the primary search results for both academic and grey literature to extract the first set of the edge-to-cloud offloading tools. Two authors assessed each source independently considering mentioned criteria to make the decision if the search result should be included or not. For those which are included, if they found the tool in the search result, they extract the name of the tool and added in a separate column. Based on that, we created the first list of the tools where at least one of the authors agreed on its inclusion. At this stage, 338 tools were selected.


% \subsection{Search results evaluation}

%  All the tools in the first list moved to a new sheet for the final evaluation. Two authors separately assessed each source which is related to a tool considering research questions and inclusion and exclusion criteria. When both agreed on exclusion, the tool became rejected. However, for the results with disagreement, we discussed the evaluation with third person to make the final decision. As a result, we selected 94 tools. 



% \subsection{Data extraction and synthesis}  

% Based on the RQs, we extracted the information about the final tools on a structured review spreadsheet.

% First, we extracted the source of the tool with its main reference, after we focused on the different characteristics explicitly declared for each tool, at last we extracted also information regarding the targeted environment of the tool.

% \subsection{Final pool of sources}

% After performing the data extraction and synthesis we focused on one of the characteristics extracted during the previous stage: \textit{Tool Type}.
% In the previous stage we had 3 possible outcomes for the Tool Type characteristic, namely Commercial, Open Source and Research Prototype. As a quality check, we included two more exclusion criteria:
% \begin{itemize}
%     \item Quality Exclusion Criteria 1: Tool not available online
%     \item Quality Exclusion Criteria 2: Open Source Tool with less than 100 stars in GitHub.
% \end{itemize}
% This would result in checking every single tool marked as Research Prototype and categorizing it as Commercial or Open Source. Whenever a tool would not respect any of the Quality Exclusion Criteria it would be automatically excluded. 

% After the Quality Check the final selected tools were 42.  










==> Sections/Study_results_Backup.tex <==
\section{Study Results}
\label{sec:StudyResults}


% Please add the following required packages to your document preamble:




In this section, we present the results of our MLR study guided by the research questions stated in section \ref{sec:ResearchQuestions}. %These results are based on data extracted from 40 selected sources including 10 academic paper and 30 grey literature sources. Among the tools which are found from the academic literature, 8 of them are in common with grey literature sources. For each research question, we describe the context followed by relevant results.

\subsection{Edge-to-cloud offloading tools (RQ1)}

\emph{Description}. To answer RQ1, we found out the tools that have the capability to offload the computational tasks in the cloud continuum. 

\begin{table}[]
\caption{Tools categorization based on where they offload}
\centering
\adjustbox{max width=0.8\textwidth}{
\begin{tabular}{|l||l|l|}
\toprule													
\rowcolor{black} \textcolor{white}{\textbf{		Tool Name	}}	&	\textcolor{white}{\textbf{	edge-to-cloud	}}	&	\textcolor{white}{\textbf{	edge-only	}}	\\	\midrule
\rowcolor{gray10}		Amazon EKS		&				&		x		\\	
		Ambassador Edge Stack		&				&		x		\\	
\rowcolor{gray10}		Apache Airflow		&		x		&				\\	
		APEX		&		x		&				\\	
\rowcolor{gray10}		Aruba ESP		&		x		&				\\	
		Avassa		&				&		x		\\	
\rowcolor{gray10}		AWS IoT GreenGrass		&		x		&				\\	
		AWS Wavelength		&		x		&				\\	
\rowcolor{gray10}		Azure stack Edge		&		x		&				\\	
		Baetyl		&				&		x		\\	
\rowcolor{gray10}		Cloudify		&				&		x		\\	
		Docker Swarm		&		x		&				\\	
\rowcolor{gray10}		Eclipse ioFog 2.0		&		x		&				\\	
		EdgeCloudSim		&		x		&				\\	
\rowcolor{gray10}		eKuiper		&			x	&				\\	
		FogFlow		&		x		&				\\	
\rowcolor{gray10}		Home edge orchesterator		&		x		&				\\	
		Intel Smart Edge		&		x		&				\\	
\rowcolor{gray10}		k0s		&		x		&				\\	
		K3s		&		x		&				\\	
\rowcolor{gray10}		KubeEdge		&		x		&				\\	
		KubeFed		&		x		&				\\	
\rowcolor{gray10}		Kubernetes		&		x		&				\\	
		MicroK8S		&		x		&				\\	
\rowcolor{gray10}		Microsoft’s Azure IoT Edge		&		x		&				\\	
		Nearby One		&		x		&				\\	
\rowcolor{gray10}		Nomad		&		x		&				\\	
		NEBULA		&		x		&				\\	
\rowcolor{gray10}		Nuvlabox (NuvlaEdge)		&		x		&				\\	
		ONAP		&		x		&				\\	
\rowcolor{gray10}		Open horizon		&		x		&				\\	
		Open Stack Starlingx		&		x		&				\\	
\rowcolor{gray10}		OpenNebula		&		x		&				\\	
		OpenShift		&		x		&				\\	
\rowcolor{gray10}		Openstack		&		x		&				\\	
		OpenYurt		&		x		&				\\	
\rowcolor{gray10}		Ormuco		&				&		x		\\	
		Saguna		&		x		&				\\	
\rowcolor{gray10}		Windriver Studio		&		x		&				\\	
		Zededa		&		x		&				\\
\bottomrule
\end{tabular}
}
\label{table:off}
\end{table}

\emph{Results}. The main objective of task offloading is to optimize offloading of the computational tasks from end user device to a remote site under specific constraints. This process consists of three main parts which are (i) various hardware components, such as end user devices and Edge/Cloud devices, (ii) multiple computing processes, including task splitting and computational processing either locally or remotely and (iii) networking components for transferring data between the hardware components involved \cite{saeik2021task}.
Out of the 40 retrieved tools, 23 have a commercial license, 17 an Open Source License. Table \ref{tab:license} illustrates the main URL of each tool and its kind of license.

As discussed in section 2.2., based on where the tasks are executed, there are different types of task offloading. According to the final list of selected tools, we identify two types of offloading; {\em edge-to-cloud} and {\em edge-to-edge only}. As it is illustrated in Table \ref{table:off}, from the 40 tools, 6 of them are offloading the tasks only on the edge, while 34 tool can offload the tasks to the cloud.


\subsection{Tools characteristics (RQ2)}

\emph{Description}. To answer RQ2, we extracted the characteristics of the tools in the cloud continuum. 

\emph{Results}. We extracted characteristics of the identified tools and their alternatives, and grouped them into the following categories:
We identified 10 global categories:
\begin{itemize}

     \item \textbf{Offloading:} tools used to perform different kinds of offloading as introduced in Section~\ref{sec:offloading}.

    % Offloading refers to the process of transferring a computational task from one device to another, typically from a client device to a remote server or cloud-based infrastructure. Offloading is often used in mobile computing or edge computing scenarios where the client device has limited computational resources, and the server or cloud infrastructure can provide additional processing power and storage. The goal of offloading is to improve the performance of the client device and reduce its energy consumption.
    

    \item \textbf{Orchestration:} tools performing Orchestration. Tools that are capable of "managing, automating and coordinating the flow of resources between multiple types of devices, infrastructure, and network domains at the edge of a network" \cite{orch}.

    %In the context of distributed computing, orchestration is the process of coordinating multiple services and resources to automate a workflow or a task. It involves the use of an orchestration tool or framework that automates the deployment, scaling, and management of containerized applications, microservices, or other components in a distributed system. The goal of orchestration is to ensure that the various components of the system work together seamlessly to achieve the desired outcome.
    \item \textbf{Workflow Management:} tools used to manage the workflow and tasks assignable.
    \item \textbf{Proprietary Container:} tools that allow to create containerized applications.
    \item \textbf{Deployment:} tools used to managing and deploying containerized and non-containerized applications across the cloud continuum. 
    %perform large-scale deployments. 
    \item \textbf{Kubernetes Distribution:} different distributions of Kubernetes designed to provide an out-of-the-box solution for deploying Kubernetes and managing containerized workloads.
    \item \textbf{Kubernetes Extension:} additional components that extend the core functionality of Kubernetes. These extensions are developed and added by third-party. Moreover, are designed to enhance the functionality of Kubernetes and provide additional capabilities for managing complex workloads.
    %tools that perform management by extending Kubernetes functionalities. 
    \item \textbf{Simulator:} tools used to simulate specific environments for testing. Such environments are useful when performing tests among different simulated entity and devices.
    \item \textbf{End2End (E2E) Service:} set of functionalities composed of multiple tools used to automate the full lifecycle of the devices along the cloud continuum. Such tools work together seamlessly to provide the desired functionality. The goal of an end-to-end service is to provide a complete solution to a specific problem or set of problems.
    \item \textbf{Platform:} complete software environment that provides a set of services and tools for developing, deploying, and managing distributed applications. The goal of a platform is to provide a high-level abstraction of the underlying infrastructure, making it easier for developers to build and deploy distributed applications.
    

    
\end{itemize}
The mapping of each different tool to the different categories is depicted in Table~\ref{tab:char}.


\begin{table}[]
\caption{Tools characteristics}
\centering
\adjustbox{max width=0.85\textwidth}{
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|}
\rowcolor{black} \textcolor{white}{\textbf{		Tool Name	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Offloading}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Orchestration}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Workflow Management}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Proprietary Container}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Deployment}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Kubernetes Distribution}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Kubernetes Extension}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Simulator}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{E2E Service}}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Platform}}}	\\	\midrule
\rowcolor{gray10}		Amazon EKS		&					&					&					&					&					&					&			x		&					&					&					\\	
		Ambassador Edge Stack		&					&					&					&					&					&					&			x		&					&					&					\\	
\rowcolor{gray10}		Apache Airflow		&					&					&			x		&					&					&					&					&					&					&					\\	
		APEX		&					&					&					&					&					&					&					&					&			x		&					\\	
\rowcolor{gray10}		Aruba ESP		&					&					&					&					&					&					&					&					&			x		&					\\	
		Avassa		&					&					&					&					&			x		&					&					&					&					&					\\	
\rowcolor{gray10}		AWS IoT GreenGrass		&					&					&					&					&					&					&					&					&			x		&					\\	
		AWS Wavelength		&					&					&					&					&					&					&					&					&			x		&					\\	
\rowcolor{gray10}		Azure stack Edge		&					&					&					&					&					&					&					&					&			x		&					\\	
		Baetyl		&					&					&					&					&					&					&			x		&					&					&					\\	
\rowcolor{gray10}		Cloudify		&					&					&					&					&			x		&					&					&					&					&					\\	
		Docker Swarm		&					&			x		&					&					&					&					&					&					&					&					\\	
\rowcolor{gray10}		Eclipse ioFog 2.0		&					&			x		&					&					&			x		&					&					&					&					&					\\	
		EdgeCloudSim		&					&					&					&					&					&					&					&			x		&					&					\\	
\rowcolor{gray10}		eKuiper		&					&					&			x		&					&					&					&					&					&					&					\\	
		FogFlow		&					&			x		&					&					&					&					&					&					&					&					\\	
\rowcolor{gray10}		Home edge orchesterator		&					&					&					&					&					&					&					&					&					&			x		\\	
		Intel Smart Edge		&					&					&					&					&					&					&					&					&					&			x		\\	
\rowcolor{gray10}		k0s		&					&			x		&					&					&					&			x		&					&					&					&					\\	
		K3s		&					&			x		&					&					&					&			x		&					&					&					&					\\	
\rowcolor{gray10}		KubeEdge		&					&			x		&					&					&					&			x		&					&					&					&					\\	
		KubeFed		&					&		x			&					&					&					&			x		&					&					&					&					\\	
\rowcolor{gray10}		Kubernetes		&					&			x		&					&					&					&			x		&					&					&					&					\\	
		MicroK8S		&			x		&					&					&					&					&					&					&					&					&					\\	
\rowcolor{gray10}		Microsoft’s Azure IoT Edge		&					&					&					&					&					&					&					&					&			x		&					\\	
		Nearby One		&					&			x		&					&					&					&					&					&					&					&					\\	
\rowcolor{gray10}		Nomad		&					&			x		&					&			x		&					&					&					&					&					&			x		\\	
		NEBULA		&					&			x		&					&			x		&					&					&					&					&					&			x		\\	
\rowcolor{gray10}		Nuvlabox (NuvlaEdge)		&					&					&					&					&					&					&					&					&					&			x		\\	
		ONAP		&					&			x		&					&					&					&					&					&					&					&					\\	
\rowcolor{gray10}		Open horizon		&					&					&					&					&					&					&					&					&					&			x		\\	
		Open Stack Starlingx		&					&					&					&					&			x		&					&					&					&					&					\\	
\rowcolor{gray10}		OpenNebula		&					&					&					&					&					&					&					&					&					&			x		\\	

		OpenShift		&					&					&					&					&					&					&					&					&					&			x		\\	
\rowcolor{gray10}		Openstack		&					&					&					&					&					&					&					&					&					&			x		\\	
		OpenYurt		&					&					&					&					&					&					&					&					&					&			x		\\	
\rowcolor{gray10}		Ormuco		&					&					&					&					&					&					&					&					&			x		&			x		\\	
		Saguna		&					&					&					&					&					&					&					&					&					&			x		\\	
\rowcolor{gray10}		Windriver Studio		&					&					&					&					&					&					&					&					&					&			x		\\	
		Zededa		&					&					&					&					&					&					&					&					&					&			x		\\	
\bottomrule
\end{tabular}
}
\label{tab:char}
\end{table}

\begin{comment}
\begin{table}[]
\caption{Tools characteristics}
\centering
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|}
\rowcolor{black} \textcolor{white}{\textbf{		Tool Name	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Orchestration}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Offloading}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Kubernetes Extensions}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Deployment}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Simulator}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{E2E Service}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Proprietary Container}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Kubernetes Distribution }	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Workflow Management}	}}	&	\textcolor{white}{\textbf{	\rotatebox{90}{Platform}	}}	\\	\midrule
		Akraino LFEdge		&				&		x		&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Amazon EKS		&				&				&		x		&				&				&				&				&				&				&				\\	
		Ambassador Edge Stack		&				&				&		x		&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Apache Airflow		&				&				&				&				&				&				&				&				&		x		&				\\	
		APEX		&				&				&				&				&				&		x		&				&				&				&				\\	
\rowcolor{gray10}		Aruba ESP		&				&				&				&				&				&		x		&				&				&				&				\\	
		Avassa		&				&				&				&		x		&				&				&				&				&				&				\\	
\rowcolor{gray10}		AWS IoT GreenGrass		&				&				&				&				&				&		x		&				&				&				&				\\	
		AWS Wavelength		&				&				&				&				&				&		x		&				&				&				&				\\	
\rowcolor{gray10}		Azure stack Edge		&				&				&				&				&				&		x		&				&				&				&				\\	
		Baetyl		&				&				&		x		&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Cloudify		&				&				&				&		x		&				&				&				&				&				&				\\	
		Docker Swarm		&		x		&				&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Eclipse ioFog 2.0		&		x		&				&				&		x		&				&				&				&				&				&				\\	
		EdgeCloudSim		&				&				&				&				&		x		&				&				&				&				&				\\	
\rowcolor{gray10}		eKuiper		&				&				&				&				&				&				&				&				&		x		&				\\	
		FogFlow		&		x		&				&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Home edge orchesterator		&				&				&				&				&				&				&				&				&				&		x		\\	
		Intel Smart Edge		&				&				&				&				&				&				&				&				&				&		x		\\	
\rowcolor{gray10}		k0s		&				&				&				&				&				&				&				&		x		&				&				\\	
		K3s		&				&				&				&				&				&				&				&		x		&				&				\\	
\rowcolor{gray10}		KubeEdge		&				&				&				&				&				&				&				&		x		&				&				\\	
		KubeFed		&				&				&				&				&				&				&				&		x		&				&				\\	
\rowcolor{gray10}		Kubernetes		&				&				&				&				&				&				&				&		x		&				&				\\	
		MicroK8S		&				&		x		&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Microsoft’s Azure IoT Edge		&				&				&				&				&				&		x		&				&				&				&				\\	
		Nearby One		&		x		&				&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Nomad		&		x		&				&				&				&				&				&		x		&				&				&		x		\\	
		NEBULA		&		x		&				&				&				&				&				&		x		&				&				&		x		\\	
\rowcolor{gray10}		Nuvlabox (NuvlaEdge)		&				&				&				&				&				&				&				&				&				&		x		\\	
		ONAP		&		x		&				&				&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		Open horizon		&				&				&				&				&				&				&				&				&				&		x		\\	
		Open Stack Starlingx		&				&				&				&		x		&				&				&				&				&				&				\\	
\rowcolor{gray10}		OpenNebula		&				&				&				&				&				&				&				&				&				&		x		\\	
		Openness		&		x		&				&		x		&				&				&				&				&				&				&				\\	
\rowcolor{gray10}		OpenShift		&				&				&				&				&				&				&				&				&				&		x		\\	
		Openstack		&				&				&				&				&				&				&				&				&				&		x		\\	
\rowcolor{gray10}		OpenYurt		&				&				&				&				&				&				&				&				&				&		x		\\	
		Ormuco		&				&				&				&				&				&		x		&				&				&				&		x		\\	
\rowcolor{gray10}		Saguna		&				&				&				&				&				&				&				&				&				&		x		\\	
		Windriver Studio		&				&				&				&				&				&				&				&				&				&		x		\\	
\rowcolor{gray10}		Zededa		&				&				&				&				&				&				&				&				&				&		x		\\	
\bottomrule
\end{tabular}
}
\label{tab:char}
\end{table}

\end{comment}



\subsection{Tools environment (RQ3)}

\emph{Description}. To answer RQ3, we identified the target environment for each tool. 

\emph{Results}. We categorized the different tools based on the main environment they target. We identified 4 different alternatives:
\begin{itemize}
    \item \textbf{Agnostic:} tools created to run seamlessly on different entities among the cloud continuum. We identified 29 tools which are agnostic.
    \item \textbf{Cloud Infrastructure:} tools that target the Cloud as the main environment to be run. Out of 40 final tools, 6 of them could be run at cloud infrastructures.
    \item \textbf{Edge Node:} tools made to run on Edge Devices. We found 5 tools that their main environment are edge nodes.
    \item \textbf{Far Edge:} tools targeting the deployment on those devices which reside in the Far Edge and therefore have lower computation capabilities. Based on our results, only 1 tool made to run on far edge.
\end{itemize}
Table~\ref{tab:env} maps each different tool to its targeted environment.
\begin{table}[]
\caption{Targeted environment for the specific tools}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{|l||l|l|l|l|}
\toprule																					
\rowcolor{black} \textcolor{white}{\textbf{		Tool	}}	&	\textcolor{white}{\textbf{	Agnostic	}}	&	\textcolor{white}{\textbf{	Cloud	}}	&	\textcolor{white}{\textbf{	Edge	}}	&	\textcolor{white}{\textbf{	Far	}}	\\	
\rowcolor{black} \textcolor{white}{\textbf{		Name	}}	&	\textcolor{white}{\textbf{		}}	&	\textcolor{white}{\textbf{	Infrastructure	}}	&	\textcolor{white}{\textbf{	Node	}}	&	\textcolor{white}{\textbf{	Edge	}}	\\	\midrule

\rowcolor{gray10}		Amazon EKS		&		x		&				&				&				\\	
		Ambassador Edge Stack		&		x		&				&				&				\\	
\rowcolor{gray10}		Apache Airflow		&		x		&				&				&				\\	
		APEX		&		x		&				&				&				\\	
\rowcolor{gray10}		Aruba ESP		&				&		x		&				&				\\	
		Avassa		&		x		&				&				&				\\	
\rowcolor{gray10}		AWS IoT GreenGrass		&				&				&		x		&				\\	
		AWS Wavelength		&				&				&		x		&				\\	
\rowcolor{gray10}		Azure stack Edge		&				&		x		&				&				\\	
		Baetyl		&		x		&				&				&				\\	
\rowcolor{gray10}		Cloudify		&		x		&				&				&				\\	
		Docker Swarm		&		x		&				&				&				\\	
\rowcolor{gray10}		Eclipse ioFog 2.0		&		x		&				&				&				\\	
		EdgeCloudSim		&				&		x		&				&				\\	
\rowcolor{gray10}		eKuiper		&				&				&				&		x		\\	
		FogFlow		&		x		&				&				&				\\	
\rowcolor{gray10}		Home edge orchesterator		&		x		&				&				&				\\	
		Intel Smart Edge		&				&		x		&				&				\\	
\rowcolor{gray10}		k0s		&		x		&				&				&				\\	
		K3s		&		x		&				&				&				\\	
\rowcolor{gray10}		KubeEdge		&		x		&				&				&				\\	
		KubeFed		&		x		&				&				&				\\	
\rowcolor{gray10}		Kubernetes		&		x		&				&				&				\\	
		MicroK8S		&		x		&				&				&				\\	
\rowcolor{gray10}		Microsoft’s Azure IoT Edge		&		x		&				&				&				\\	
		Nearby One		&				&				&		x		&				\\	
\rowcolor{gray10}		Nomad		&		x		&				&				&				\\	
		NEBULA		&		x		&				&				&				\\	
\rowcolor{gray10}		Nuvlabox (NuvlaEdge)		&		x		&				&				&				\\	
		ONAP		&				&		x		&				&				\\	
\rowcolor{gray10}		Open horizon		&				&				&		x		&				\\	
		Open Stack Starlingx		&				&		x		&				&				\\	
\rowcolor{gray10}		OpenNebula		&		x		&				&				&				\\	
		OpenShift		&		x		&				&				&				\\	
\rowcolor{gray10}		Openstack		&		x		&				&				&				\\	
		OpenYurt		&		x		&				&				&				\\	
\rowcolor{gray10}		Ormuco		&		x		&				&				&				\\	
		Saguna		&				&				&		x		&				\\	
\rowcolor{gray10}		Windriver Studio		&		x		&				&				&				\\	
		Zededa		&		x		&				&				&				\\	
\bottomrule
\end{tabular}
}
\label{tab:env}
\end{table}
